Pest-Thinker: Learning to Think and Reason like Entomologists via Reinforcement Learning

Pest-induced crop losses pose a major threat to global food security and sustainable agricultural development. While recent advances in Multimodal Large Language Models (MLLMs) have shown strong potential for visual understanding and smart agriculture, their direct application to pest recognition remains limited due to the domain's unique challenges such as high inter-species complexity, intra-species variability, and the scarcity of expert-annotated data. In this work, we introduce Pest-Thinker, a knowledge-driven reinforcement learning (RL) framework that enables MLLMs to reason over fine-grained pest morphology. We first construct two high-definition pest benchmarks, QFSD and AgriInsect, comprising diverse species and expert-annotated morphological traits. Leveraging these datasets, we synthesize Chain-of-Thought (CoT) reasoning trajectories to facilitate structured learning of pest-specific visual cues through Supervised Fine-Tuning (SFT). Subsequently, we employ Group Relative Policy Optimization (GRPO) with a novel feature reward that guides the model to focus on observable morphological evidence, assessed by an LLM-as-a-Judge strategy. Extensive experiments demonstrate that Pest-Thinker substantially improves both in-domain and out-of-domain morphological understanding, marking a step toward expert-level visual reasoning for intelligent agricultural pest analysis. The datasets and source code are available upon acceptance.

==> sec/3_datapipline.tex <==
% \section{Data Pipeline}

%To enable MLLMs to acquire human-like reasoning abilities for agricultural pest identification, it is essential to construct a high-quality, cognitively grounded image CoT dataset. The PEST CoT (Chain-of-Thought) Dataset addresses this need by providing a comprehensive collection of agricultural pest identification samples with structured reasoning processes. This dataset incorporates a cognition-inspired pipeline that integrates structured pest knowledge and cognitive prompting strategies to generate high-quality chain-of-thought annotations for fine-grained species-level pest classification tasks.

% \subsection{Data}

%We extensively collect pest identification data covering diverse agricultural pest species across multiple morphological states. The dataset , QFSD and AgriInsect, comprising a total of 200 pest species with more than 4,000 annotated test samples. Each sample follows a standardized multiple-choice question format with four options (A, B, C, D), where each option represents a pest species identified by its Latin scientific name. The dataset emphasizes fine-grained species-level identification, requiring models to distinguish between visually similar pests based on subtle morphological features such as wing patterns, body coloration, and other distinguishing characteristics. Additionally, the dataset includes 200 pest species with multiple morphological states (e.g., adult, larva, nymph, pupa, egg), enabling comprehensive evaluation scenarios where models must recognize the same pest species across different developmental stages.

%\subsection{Expert-Knowledge-Injected CoT Generation}

% To construct a high-quality CoT dataset for agricultural pest identification, we propose an automated pipeline for generating cognitively grounded CoT annotations. As illustrated in Fig.~\ref{fig:cot-pipeline}, the pipeline comprises three major stages: structured pest knowledge representation, cognitively inspired CoT generation, and quality filtering.

%\subsubsection{Structured Pest Knowledge Representation}

% \hspace{0.422cm}For each pest category, we extract and organize core visual features from the agricultural pest knowledge base to create structured knowledge representations. The knowledge base provides comprehensive information including Chinese names, Latin names, morphological features, life stages, and taxonomic classifications. We structure this knowledge into eight key feature categories specifically designed for image recognition: (1) Overall Body Size and Shape, (2) Head Features (Shape, Color, Compound Eyes, Antennae, etc.), (3) Thorax Features (Pronotum, Scutellum, etc.), (4) Abdomen Features (Shape, Color, Segments, etc.), (5) Wing Features (Shape, Color, Patterns, Transparency, etc.), (6) Leg Features (Color, Morphology, Special Structures, etc.), (7) Body Surface Features (Hair, Luster, Texture, etc.), and (8) Special Markings (Spots, Stripes, Special Structures, etc.). Each feature category is carefully curated to contain only appearance features observable through images, excluding biological characteristics such as habits, distribution, or host information. This structured knowledge, denoted as $K_p$ for pest $p$, serves as domain-specific knowledge to be injected into the prompting process.

% \subsubsection{Cognitively Inspired Prompting Strategy}

% \hspace{0.422cm}Given the structured knowledge representation $K_p$ and a corresponding pest image $I$ with multiple-choice question $q$, we invoke Qwen2.5VL:72B, a reasoning-capable MLLM, to generate initial CoT annotations through a cognitively inspired prompting strategy. Specifically, the prompt $P_{\text{cog}}$ consists of a composite structure that mimics human cognitive processing:

% \begin{itemize}
%     \item \textbf{System Prompt}: Instructs the model to act as an expert entomologist identifying agricultural pests from field images, emphasizing natural language description of striking features and systematic comparison with options.
%     \item \textbf{User Prompt}: Incorporates the pest knowledge through structured feature descriptions, presenting the multiple-choice question with options, and explicitly requesting the model to ``think about this question as if you were a human pondering deeply''. The prompt encourages the use of natural language thought expressions such as ``let me think'', ``wait'', ``Hmm'', ``oh, I see'', and ``let's break it down'', and includes self-reflection or verification in the reasoning process.
% \end{itemize}

% The initial CoT is generated as:
% \begin{equation}
% \text{CoT}_I^{(0)} = \text{MLLM}(q, K_p, I, P_{\text{cog}}),
% \end{equation}
% where the MLLM (specifically Qwen2.5VL:72B) directly processes the pest image $I$ along with the structured knowledge $K_p$ and question $q$. The model is instructed to provide detailed reasoning within the \texttt{<think>} tag, and the final answer within the \texttt{<answer>} tag. Additionally, the reasoning process should include a high-level category classification (e.g., beetle, moth, bug) within the \texttt{<General>} tag.

% \subsubsection{Quality Filtering and Validation}

% \hspace{0.422cm}To ensure the factual correctness and visual grounding of the resulting CoT annotations, we apply a filtering stage that validates the generated reasoning against ground-truth labels. For multiple-choice tasks with clear ground-truth answers, we directly exclude samples with incorrect final answers. Additionally, we verify that the reasoning process systematically analyzes morphological features and compares them against each option, ensuring that the CoT demonstrates genuine reasoning rather than surface-level pattern matching. This filtering process ensures that the resulting CoT dataset maintains high quality and factual reliability.

% \subsection{Data Analysis}

% \hspace{0.422cm}Figure~\ref{fig:cot-analysis} presents an analysis of the CoT annotations in the PEST CoT Dataset. As shown in Fig.~\ref{fig:cot-analysis}(a), the reasoning processes exhibit a broad distribution of token lengths with an average of approximately 400.9 tokens, primarily concentrated in the 300-500 token range. The distribution approximates a normal distribution with a relatively small standard deviation, indicating consistent reasoning depth across samples. Additionally, the word cloud in Fig.~\ref{fig:cot-analysis}(b) reveals that CoTs are dominated by entomological terminology including morphological feature descriptors such as ``wings'', ``body'', ``antennae'', ``thorax'', color vocabulary (``black'', ``yellow'', ``brown'', ``green''), and shape descriptions (``slender'', ``elongated'', ``triangular''). The lexical profile reflects an emphasis on systematic morphological analysis, feature comparison, and logical reasoning—key characteristics of expert-level pest identification. These results highlight that the PEST CoT Dataset offers substantial expressiveness in reasoning depth and aligns closely with the demands of real-world agricultural pest identification tasks, providing a strong foundation for training MLLMs with advanced reasoning capabilities.

% \subsection{Evaluation and Benchmarking}

% \hspace{0.422cm}The PEST CoT Dataset serves as a standardized benchmark for evaluating vision-language models on agricultural pest identification tasks. The explicit reasoning annotations enable not only accuracy-based evaluation but also comprehensive assessment of reasoning quality, feature extraction correctness, logical consistency, and morphological analysis depth in the identification process. The structured format with standardized tags (\texttt{<think>}, \texttt{<answer>}, \texttt{<General>}) supports automated evaluation pipelines, facilitating large-scale model comparison and performance analysis across different model architectures and training paradigms. Additionally, the multi-morphological support enables evaluation of model robustness across different developmental stages of the same pest species, providing insights into the generalization capabilities of learned representations.


